Stealthy Coverage Control for Human-enabled Real-Time 3D Reconstruction

In this paper, we propose a novel semi-autonomous image sampling strategy, called stealthy coverage control, for human-enabled 3D structure reconstruction. The present mission involves a fundamental problem: while the number of images required to accurately reconstruct a 3D model depends on the structural complexity of the target scene to be reconstructed, it is not realistic to assume prior knowledge of the spatially non-uniform structural complexity. We approach this issue by leveraging human flexible reasoning and situational recognition capabilities. Specifically, we design a semi-autonomous system that leaves identification of regions that need more images and navigation of the drones to such regions to a human operator. To this end, we first present a way to reflect the human intention in autonomous coverage control. Subsequently, in order to avoid operational conflicts between manual control and autonomous coverage control, we develop the stealthy coverage control that decouples the drone motion for efficient image sampling from navigation by the human. Simulation studies on a Unity/ROS2-based simulator demonstrate that the present semi-autonomous system outperforms the one without human interventions in the sense of the reconstructed model quality.

==> latexmkrc <==
#!/usr/bin/env perl
##============================================================================##
## description  latexmk config file
## author       Ryotaro Onuki (GitHub: kerikun11)
## created_at   2019.01.25
## modified_at  2020.02.10
##============================================================================##
## latex commands; %S: src, %O: option, %D: dest, %B: src without extension
$pdflatex   = 'lualatex -f --synctex=1 --interaction=nonstopmode --halt-on-error --file-line-error %O %S';
$max_repeat = 4;
# $latex      = 'platex -synctex=1 -halt-on-error -interaction=nonstopmode %O %S';
# $bibtex     = 'pbibtex -kanji=utf8 %O %B';
# $biber      = 'biber --bblencoding=utf8 -u -U --output_safechars';
# $dvipdf     = 'dvipdfmx %O -o %D %S';
# $makeindex  = 'mendex %O -o %D %S';
# $bibtex_use = 2;
##============================================================================##
## pdf mode
$pdf_mode   = 1; # 0: none, 1: pdflatex, 2: ps2pdf, 3: dvipdf
##============================================================================##
## output directory
$aux_dir    = "build";
$out_dir    = "build";
##============================================================================##
## configure theme path
ensure_path('TEXINPUTS', './theme');
##============================================================================##
## avoid log linebreaks; see https://tex.stackexchange.com/questions/384133/
$ENV{max_print_line} = $log_wrap = 10000;
##============================================================================##
## viewer settings
$pvc_view_file_via_temporary = 0;
if ($^O eq 'darwin') {
    # OSX
    $pdf_previewer = 'open -a Preview';
} elsif ($^O eq 'linux') {
    # Linux
    $pdf_previewer = 'evince';
} else {
    # Windows
    $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance %O %S';
}
##============================================================================##
$bibtex = 'pbibtex';
